Computing rank-revealing factorizations of matrices stored out-of-core

This paper describes efficient algorithms for computing rank-revealing factorizations of matrices that are too large to fit in RAM, and must instead be stored on slow external memory devices such as solid-state or spinning disk hard drives (out-of-core or out-of-memory). Traditional algorithms for computing rank revealing factorizations, such as the column pivoted QR factorization, or techniques for computing a full singular value decomposition of a matrix, are very communication intensive. They are naturally expressed as a sequence of matrix-vector operations, which become prohibitively expensive when data is not available in main memory. Randomization allows these methods to be reformulated so that large contiguous blocks of the matrix can be processed in bulk. The paper describes two distinct methods. The first is a blocked version of column pivoted Householder QR, organized as a "left-looking" method to minimize the number of write operations (which are more expensive than read operations on a spinning disk drive). The second method results in a so called UTV factorization which expresses a matrix $A$ as $A = U T V^*$ where $U$ and $V$ are unitary, and $T$ is triangular. This method is organized as an algorithm-by-blocks, in which floating point operations overlap read and write operations. The second method incorporates power iterations, and is exceptionally good at revealing the numerical rank; it can often be used as a substitute for a full singular value decomposition. Numerical experiments demonstrate that the new algorithms are almost as fast when processing data stored on a hard drive as traditional algorithms are for data stored in main memory. To be precise, the computational time for fully factorizing an $n\times n$ matrix scales as $cn^{3}$, with a scaling constant $c$ that is only marginally larger when the matrix is stored out of core.

==> figs/fig_dispatcher.tex <==


\begin{figure}
\begin{subfigure}{.6\linewidth}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\multicolumn{1}{|c|}{Operation} &
\multicolumn{3}{c|}{Operands} \\ \cline{2-4}
& \multicolumn{2}{c|}{In} & In/Out \\
\hline
Generate\_normal\_random & & & $G_0$ \checkmark \\
\hline
Generate\_normal\_random & & & $G_1$ \checkmark \\
\hline
Gemm\_tn\_oz: $C = A^* B$ & $A_{00}$ \checkmark & $G_{0}$ & $Y_0$ \checkmark \\
\hline
Gemm\_tn\_oz: $C = A^* B$ & $A_{01}$ \checkmark & $G_{0}$ & $Y_1$ \checkmark \\
\hline
Gemm\_tn\_oo: $C = C + A^* B$ & $A_{10}$ \checkmark & $G_{1}$ & $Y_{0}$ \\
\hline
Gemm\_tn\_oo: $C = C + A^* B$ & $A_{11}$ \checkmark & $G_{1}$ & $Y_{1}$ \\
\hline
Comp\_dense\_QR & & & $Y_{0}$, $S_0$ \checkmark \\
\hline
Copy & $Y_{0}$ & & $Y_0$ \checkmark \\
\hline
Comp\_td\_QR & & & $Y_0$, $Y_1$, $S_1$ \checkmark \\
\hline
Apply\_right\_Q\_of\_dense\_QR & $Y_0$ & $S_0$ & $A_{00}$ \checkmark \\
\hline
Apply\_right\_Q\_of\_dense\_QR & $Y_0$ & $S_0$ & $A_{10}$ \checkmark \\
\hline
Apply\_right\_Q\_td\_QR & $Y_1$ & $S_1$ & $A_{00}, A_{01}$ \checkmark \\
\hline
Apply\_right\_Q\_td\_QR & $Y_1$ & $S_1$ & $A_{10}, A_{11}$ \checkmark \\
\hline
\end{tabular}
\minusvs
\caption{First half of the original table}
\vs

\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\centering
\begin{tabular}{| c | c | c |}
\hline
\multicolumn{3}{| c |}{Operands} \\
\cline{1-3}
\multicolumn{2}{| c |}{In} & In/Out \\
\hline
& & \\
\hline
& & \\
\hline
$A_{00}$ \checkmark & $G_{0}$ \checkmark & $Y_0$ \checkmark \\
\hline
$A_{01}$ \checkmark & $G_{0}$ \checkmark & $Y_1$ \checkmark \\
\hline
$A_{10}$ \checkmark & $G_{1}$ \checkmark & $Y_{0}$ \\
\hline
$A_{11}$ \checkmark & $G_{1}$ \checkmark & $Y_{1}$ \\
\hline
& & $Y_{0}$, $S_0$ \checkmark \\
\hline
$Y_{0}$ & & $Y_0$ \checkmark \\
\hline
& & $Y_0$, $Y_1$, $S_1$ \checkmark \\
\hline
$Y_0$ & $S_0$ & $A_{00}$ \checkmark \\
\hline
$Y_0$ & $S_0$ & $A_{10}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{00}, A_{01}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{10}, A_{11}$ \checkmark \\
\hline
\end{tabular}
\minusvs
\caption{After second operation}
\vs

\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\centering
\begin{tabular}{| c | c | c |}
\hline
\multicolumn{3}{| c |}{Operands} \\
\cline{1-3}
\multicolumn{2}{| c |}{In} & In/Out \\
\hline
& & \\
\hline
& & \\
\hline
 & & \\
\hline
 & & \\
\hline
$A_{10}$ \checkmark & $G_{1}$ \checkmark & $Y_{0}$ \checkmark \\
\hline
$A_{11}$ \checkmark & $G_{1}$ \checkmark & $Y_{1}$ \checkmark \\
\hline
& & $Y_{0}$, $S_0$ \checkmark \\
\hline
$Y_{0}$ & & $Y_0$ \checkmark \\
\hline
& & $Y_0$, $Y_1$, $S_1$ \checkmark \\
\hline
$Y_0$ & $S_0$ & $A_{00}$ \checkmark \\
\hline
$Y_0$ & $S_0$ & $A_{10}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{00}, A_{01}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{10}, A_{11}$ \checkmark \\
\hline
\end{tabular}
\minusvs
\caption{After fourth operation}
\vs

\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\centering
\begin{tabular}{| c | c | c |}
\hline
\multicolumn{3}{| c |}{Operands} \\
\cline{1-3}
\multicolumn{2}{| c |}{In} & In/Out \\
\hline
& & \\
\hline
& & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
& & $Y_{0}$ \checkmark , $S_0$ \checkmark \\
\hline
$Y_{0}$ & & $Y_0$ \checkmark \\
\hline
& & $Y_0$, $Y_1$ \checkmark , $S_1$ \checkmark \\
\hline
$Y_0$ & $S_0$ & $A_{00}$ \checkmark \\
\hline
$Y_0$ & $S_0$ & $A_{10}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{00}, A_{01}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{10}, A_{11}$ \checkmark \\
\hline
\end{tabular}
\minusvs
\caption{After sixth operation}
\vs

\end{subfigure}
\begin{subfigure}{0.3\linewidth}
\centering
\begin{tabular}{| c | c | c |}
\hline
\multicolumn{3}{| c |}{Operands} \\
\cline{1-3}
\multicolumn{2}{| c |}{In} & In/Out \\
\hline
& & \\
\hline
& & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
& & \\
\hline
$Y_{0}$ \checkmark & & $Y_0$ \checkmark \\
\hline
& & $Y_0$, $Y_1$ \checkmark , $S_1$ \checkmark \\
\hline
$Y_0$ & $S_0$ \checkmark & $A_{00}$ \checkmark \\
\hline
$Y_0$ & $S_0$ \checkmark & $A_{10}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{00}, A_{01}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{10}, A_{11}$ \checkmark \\
\hline
\end{tabular}
\minusvs
\caption{After seventh operation}
\vs

\end{subfigure}
\begin{subfigure}{0.4\linewidth}
\centering
\begin{tabular}{| c | c | c |}
\hline
\multicolumn{3}{| c |}{Operands} \\
\cline{1-3}
\multicolumn{2}{| c |}{In} & In/Out \\
\hline
& & \\
\hline
& & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
& & \\
\hline
& & \\
\hline
& & $Y_0$ \checkmark, $Y_1$ \checkmark , $S_1$ \checkmark \\
\hline
$Y_0$ \checkmark & $S_0$ \checkmark & $A_{00}$ \checkmark \\
\hline
$Y_0$ \checkmark & $S_0$ \checkmark & $A_{10}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{00}, A_{01}$ \checkmark \\
\hline
$Y_1$ & $S_1$ & $A_{10}, A_{11}$ \checkmark \\
\hline
\end{tabular}
\minusvs
\caption{After eighth operation}
\vs

\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\centering
\begin{tabular}{| c | c | c |}
\hline
\multicolumn{3}{| c |}{Operands} \\
\cline{1-3}
\multicolumn{2}{| c |}{In} & In/Out \\
\hline
& & \\
\hline
& & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
 & & \\
\hline
& & \\
\hline
& & \\
\hline
& & \\
\hline
 & & \\
\hline
 & & \\
\hline
$Y_1$ \checkmark & $S_1$ \checkmark & $A_{00} \checkmark, A_{01}$ \checkmark \\
\hline
$Y_1$ \checkmark & $S_1$ \checkmark & $A_{10} \checkmark, A_{11}$ \checkmark \\
\hline
\end{tabular}
\minusvs
\caption{After eleventh operation}
\vs
\end{subfigure}

\caption{ 
An illustration of the execution order of 
the first half (the first tasks) of \texttt{randUTV\_AB} 
for an $n \times n$ matrix using the SuperMatrix runtime system 
when the block size is $n/2$. 
A check mark `\checkmark' indicates the value is available. 
The execution order may change depending on the number of available cores 
in the system.}
\label{fig:dispatcher}
\end{figure}



==> figs/fig_qr_ab_by_columns.tex <==
%
% Figure with tasks of QR_AB.
%

% Usual element:  Usual bullet. 
\newcommand{\mybl}{\bullet}
% Usual element:  Usual bullet forced not to have surrounding lines.
\newcommand{\mybn}{\multicolumn{1}{c}{\bullet}} 
% Modified element:  Usual star. 
\newcommand{\mysl}{\star}
% Modified element:  Usual star forced not to have surrounding lines.
\newcommand{\mysn}{\multicolumn{1}{c}{\star}}
% Nullified element:  Usual cdot. 
\newcommand{\mypl}{\cdot}
% Nullified element:  Usual cdot forced not to have surrounding lines.
\newcommand{\mypn}{\multicolumn{1}{c}{\cdot}}


% Use arabic numbers for the subfigures.
\renewcommand{\thesubfigure}{\arabic{subfigure}}


\begin{figure}
%
% Subfigure 1.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|cccccc} 
\cline{1-3}
  \mysl & \mysl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mypl & \mysl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mypl & \mypl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\ 
\cline{1-3}
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
\end{array}
\]
\minusvs
\caption{After Compute\_QR( $A_{00}$ ) \newline}
\vs
\end{subfigure}
%
\hspace*{0.3cm}
%
% Subfigure 2.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|cccccc} 
\cline{1-3}
  \mysl & \mysl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mypl & \mysl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mypl & \mypl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\ 
\cline{1-3}
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\cline{1-3}
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mybn & \mybl & \mybn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\end{array}
\]
\minusvs
\caption{After Compute\_td\_\-QR( $A_{00}$, $A_{10}$ )}
\vs
\end{subfigure}
%
\hspace*{0.3cm}
%
% Subfigure 3.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|cccccc} 
\cline{1-3}
  \mysl & \mysl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mypl & \mysl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\
  \mypl & \mypl & \mysl & \mybl & \mybl & \mybl & \mybl & \mybl & \mybl \\ 
\cline{1-3}
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\cline{1-3}
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\cline{1-3}
\end{array}
\]
\minusvs
\caption{After Compute\_td\_\-QR( $A_{00}$, $A_{20}$ )}
\end{subfigure}
%
% Subfigure 4.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|ccc|ccc} 
\cline{1-6}
  \mybl & \mybl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\
  \mypl & \mybl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\
  \mypl & \mypl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\ 
\cline{1-6}
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybl \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybl \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybl \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybl \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybl \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybl \\
\end{array}
\]
\minusvs
\caption{After Apply\_left\_Qt\_of\_Den\-se\_QR( $A_{00}$, $A_{01}$ )}
\vs
\end{subfigure}
%
\hspace*{0.3cm}
%
% Subfigure 5.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|ccc|ccc} 
\cline{1-6}
  \mybl & \mybl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\
  \mypl & \mybl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\
  \mypl & \mypl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\ 
\cline{1-6}
  \mypl & \mypl & \mypl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybn \\
\cline{1-6}
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\end{array}
\]
\minusvs
\caption{After Apply\_left\_Qt\_of\_\-td\_QR( $A_{00}$, $A_{10}$, $A_{01}$, $A_{11}$ )}
\vs
\end{subfigure}
%
\hspace*{0.3cm}
%
% Subfigure 6.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|ccc|ccc} 
\cline{1-6}
  \mybl & \mybl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\
  \mypl & \mybl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\
  \mypl & \mypl & \mybl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybl \\ 
\cline{1-6}
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\cline{1-6}
  \mypl & \mypl & \mypl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybn \\
  \mypl & \mypl & \mypl & \mysl & \mysl & \mysl & \mybl & \mybl & \mybn \\
\cline{1-6}
\end{array}
\]
\minusvs
\caption{After Apply\_left\_Qt\_of\_\-td\_QR( $A_{00}$, $A_{20}$, $A_{01}$, $A_{21}$ )}
\end{subfigure}
%
% Subfigure 7.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|ccc|ccc|} 
\cline{1-3} \cline{7-9}
  \mybl & \mybl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mybl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mypl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\ 
\cline{1-3} \cline{7-9}
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\end{array}
\]
\minusvs
\caption{After Apply\_left\_Qt\_of\_Den\-se\_QR( $A_{00}$, $A_{02}$ )}
\vs
\end{subfigure}
%
\hspace*{0.3cm}
%
% Subfigure 8.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|ccc|ccc|} 
\cline{1-3} \cline{7-9}
  \mybl & \mybl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mybl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mypl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\ 
\cline{1-3} \cline{7-9}
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
\cline{1-3} \cline{7-9}
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\end{array}
\]
\minusvs
\caption{After Apply\_left\_Qt\_of\_\-td\_QR( $A_{00}$, $A_{10}$, $A_{02}$, $A_{12}$ )}
\vs
\end{subfigure}
%
\hspace*{0.3cm}
%
% Subfigure 9.
%
\begin{subfigure}{.30\linewidth}
\footnotesize
\centering
\[
\begin{array}{|ccc|ccc|ccc|} 
\cline{1-3} \cline{7-9}
  \mybl & \mybl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mybl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mypl & \mybl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\ 
\cline{1-3} \cline{7-9}
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
  \mypn & \mypl & \mypn & \mybl & \mybl & \mybn & \mybl & \mybl & \mybn \\
\cline{1-3} \cline{7-9}
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
  \mypl & \mypl & \mypl & \mybl & \mybl & \mybl & \mysl & \mysl & \mysl \\
\cline{1-3} \cline{7-9}
\end{array}
\]
\minusvs
\caption{After Apply\_left\_Qt\_of\_\-td\_QR( $A_{00}$, $A_{20}$, $A_{02}$, $A_{22}$ )}
\end{subfigure}

\caption{An illustration of the first tasks peformed by an algorithm-by-blocks 
for nullifying the first column block and updating the rest of the matrix.
The `$\bullet$' symbol represents a non-modified element by the current task,
`$\star$' represents a modified element by the current task, and
`$\cdot$' represents a nullified element by the current task
(they are shown because they store information 
about the Householder transformations that will be later used to apply them).
The continuous lines surround the blocks involved in the current task.}
\label{fig:qr_ab}
\end{figure}


